Best Axes Composition: Multiple Gyroscopes IMU Sensor Fusion to Reduce Systematic Error

In this paper, we propose an algorithm to combine multiple cheap Inertial Measurement Unit (IMU) sensors to calculate 3D-orientations accurately. Our approach takes into account the inherent and non-negligible systematic error in the gyroscope model and provides a solution based on the error observed during previous instants of time. Our algorithm, the Best Axes Composition (BAC), chooses dynamically the most fitted axes among IMUs to improve the estimation performance. We compare our approach with a probabilistic Multiple IMU (MIMU) approach, and we validate our algorithm in our collected dataset. As a result, it only takes as few as 2 IMUs to significantly improve accuracy, while other MIMU approaches need a higher number of sensors to achieve the same results.

==> _backup.tex <==
\section{Rigid Body Transformation IMU}\label{sec_rbt}


We will follow a different derivation for the equations. The difference is that instaead oif integrating sensor reading, we will calculate the derivative of poses (trajectory).
By following this derivation we will obtain the same result as explained on the background section with an additional term.


Poses are expressed as rigid body transformations $T \in SE(3)$.

\begin{equation}
\lfT{W}\rf{I}(t) = \begin{bmatrix} \lfR{W}\rf{I}(t) & \lf{W}p\rf{I}(t) \\ 
                              0 & 1 \end{bmatrix}
\label{eq_first}
\end{equation}


In order to differentiate a transformation $T \in \SE3$, we need to follow the chian rule and obtain 

\WORRIES{Should we use this chain rule? Is it better to use just well known $T^{-1} \dot T = [v, \omega]$?}

\TODO{check this, but then you can differentiate the translation components t}
\WORRIES{$V^{-1}$}
\begin{gather}
\lf{W}\dot{T}\rf{I}(t) = \frac{\partial T}{\partial \xi} \frac{\partial \xi}{\partial t} 
=\frac{\partial [R\Exp(\int_{0}^{dt}\omega(t')dt') p(t)]}{\partial \xi(i)} \\
= \begin{bmatrix} \lfR{W}\rf{I}(t)\cdot \omega(t)^{\land}  & V^{-1}\lf{W}\dot{p}\rf{I}(t) \\ 
                              0 & 1 \end{bmatrix} 
\end{gather}

\begin{equation}
\lf{W}\ddot{T}\rf{I}(t) = \begin{bmatrix} \lfR{W}\rf{I}(t) (\omega(t)^{\land})^2 + 
                        \lfR{W}\rf{I}(t) \dot{\omega}(t)^{\land} &
                        \lf{W}p\rf{I} \\ 
                              0 & 1 \end{bmatrix}
\label{eq_first}
\end{equation}

Expansion from the body frame
\begin{equation}
\dot{T} = T \cdot \lf{B}W
\label{eq_SE3_body}
\end{equation}


\begin{equation}
\frac{\partial \dot{T}}{\partial t} = \dot{T}W + T\dot{W} =
 T \cdot \lf{B}W^2 + T\cdot \lf{B}\dot{W}
\label{eq_SE3_diff}
\end{equation}

\begin{equation}
\lf{B}{W} = \begin{bmatrix} \lf{B}\omega(t)^{\land}) & \lf{B}v \\ 
                              0 & 0 \end{bmatrix}
\end{equation}

\begin{equation}
\lf{B}\dot{W} = \begin{bmatrix} 0 & \lf{B}a \\ 
                              0 & 0 \end{bmatrix}
\end{equation}

Piece-wise constant angular velocity and piece-wise constant acceleration.

An then integrate from the body twist $\lf{B}W$.


==============\\
Below is related kinematics for rigidly connected points A and B by transformation matrix $\lfT{B}\rf{A}$ that expresses frame A wrt. frame B. $\lf{A}x$ means $x$ in frame A. The same holds for B.

Poses of frames A and B in world frame (W) and their derivatives are connected by the following equations.
\\

\textbf{Zeroth derivative}
\begin{align*}
&& \lfT{W}\rf{A} &= \lfT{W}\rf{B} \lfT{B}\rf{A}\\
\\
\text{Expansion}
&& \lfR{W}\rf{A} &= \lfR{W}\rf{B} \lfR{B}\rf{A}\\
&& \lfp{W}\rf{A} &= \lfR{W}\rf{B} \lfp{B}\rf{A} + \lfp{W}\rf{B}
\end{align*}

\textbf{First derivative}

\begin{align*}
&& \lfdotT{W}\rf{A} &= \lfdotT{W}\rf{B} \lfT{B}\rf{A}\\
\\
\text{Expansion} && \lfR{W}\rf{A} [\lf{A}\omega]_\times &= \lfR{W}\rf{B} [\lf{B}\omega]_\times \lfR{B}\rf{A}\\
&& \lfR{W}\rf{A} \lf{A}v &= \lfR{W}\rf{B} ([\lf{B}\omega]_\times \lfp{B}\rf{A} + \lf{B}v)\\
\\
\text{Note 1} && [\lf{A}\omega]_\times &= \lfR{A}\rf{B} [\lf{B}\omega]_\times \lfR{B}\rf{A}\\
\text{or} && \lf{A}\omega &= \lfR{A}\rf{B} \lf{B}\omega\\
\text{Note 1} && \lf{A}v &= \lfR{A}\rf{B} ([\lf{B}\omega]_\times \lfp{B}\rf{A} + \lf{B}v)
\end{align*}

\textbf{Second derivative}
\begin{align*}
&& \lfddotT{W}\rf{A} &= \lfddotT{W}\rf{B} \lfT{B}\rf{A}\\
\\
\text{Ex}
&& \lfR{W}\rf{A} ([\lf{A}\omega]_\times^2 + [\lf{A}\dot{\omega}]_\times) &= \lfR{W}\rf{B} ([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfR{B}\rf{A}\\
%& & \lfR{W}\rf{A} ([\lf{A}\omega]_\times \lf{A}v + \lf{A}a) &= \lfR{W}\rf{B} \{([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfp{B}\rf{A} + [\lf{B}{\omega}]_\times \lf{B}v + \lf{B}a\}\\
&& \lfR{W}\rf{A} \lf{A}a &= \lfR{W}\rf{B} \{([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfp{B}\rf{A} + \lf{B}a\}\\
\\
\text{Note 1}
&& [\lf{A}\omega]_\times^2 + [\lf{A}\dot{\omega}]_\times &= \lfR{A}\rf{B} ([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfR{B}\rf{A}\\
\text{or} && \lf{A}\dot\omega &= \lfR{A}\rf{B} \lf{B}\dot\omega\\
\text{Note 2} && \lf{A}a &= \lfR{A}\rf{B} \{([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfp{B}\rf{A} + \lf{B}a\}\\
\end{align*}

$\omega, \dot \omega, v, \dot v$ IN WORLD FRAME\\

Zeroth derivative
\begin{align*}
\lfT{W}\rf{A} &= \lfT{W}\rf{B} \lfT{B}\rf{A} & \lfR{W}\rf{A} &= \lfR{W}\rf{B} \lfR{B}\rf{A}\\
& & \lfp{W}\rf{A} &= \lfR{W}\rf{B} \lfp{B}\rf{A} + \lfp{W}\rf{B}
\end{align*}

First derivative
\begin{align*}
\lfdotT{W}\rf{A} &= \lfdotT{W}\rf{B} \lfT{B}\rf{A} & [\lf{A}\omega]_\times \lfR{W}\rf{A} &= [\lf{B}\omega]_\times \lfR{W}\rf{B} \lfR{B}\rf{A}\\
& & [\lf{A}\omega]_\times \lfp{W}\rf{A} + \lf{A}v &= [\lf{B}\omega]_\times (\lfR{W}\rf{B} \lfp{B}\rf{A} + \lfp{W}\rf{B}) + \lf{B}v\\
\\
\text{Note} & & \lf{A}\omega &= \lf{B}\omega\\
\text{Note} & & \lf{A}v &= [\lf{B}\omega]_\times (\lfR{W}\rf{B} \lfp{B}\rf{A} + \lfp{W}\rf{B} - \lfp{W}\rf{A}) + \lf{B}v\\
\text{or} & & \lf{A}v &= \lf{B}v\\
\end{align*}

Second derivative
\begin{align*}
\lfddotT{W}\rf{A} &= \lfddotT{W}\rf{B} \lfT{B}\rf{A} & ([\lf{A}\omega]_\times^2 + [\lf{A}\dot{\omega}]_\times) \lfR{W}\rf{A} &= ([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfR{W}\rf{B} \lfR{B}\rf{A}\\
& & ([\lf{A}\omega]_\times^2 + [\lf{A}\dot{\omega}]_\times)\lfp{W}\rf{A} + [\lf{A}\omega]_\times \lf{A}v + \lf{A}a &= ([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) (\lfR{W}\rf{B} \lfp{B}\rf{A} + \lfp{W}\rf{B}) + [\lf{B}{\omega}]_\times \lf{B}v + \lf{B}a\\
\\
\text{Note} & & [\lf{A}\omega]_\times^2 + [\lf{A}\dot{\omega}]_\times &= [\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times\\
\text{or} & & \lf{A}\dot\omega &= \lf{B}\dot\omega\\
\text{Note} & & \lf{A}a &= \lf{B}a\\
\end{align*}
==============

But what is $\lfR{W}\rf{M}(t)$

\begin{equation}
\lf{M}\omega = \lfR{M}\rf{I}\lf{I}\omega
\label{eq_qq}
\end{equation}

For any rot m and omega belonging to SO3/so3

\begin{align}
\Exp (R \theta) = R \Exp (\theta) R^\top
\label{eq_qq}
\end{align}


\begin{equation}
\lfR{W}\rf{M}(t+\Delta t) = \lfR{W}\rf{M}(t) \Exp (\lf{M}\omega(t) \Delta t)
\label{eq_qq}
\end{equation}

\begin{equation}
\lfR{W}\rf{M}(t+\Delta t) = \lfR{W}\rf{M}(t) \lfR{M}\rf{I} \Exp (\lf{I}\omega(t) \Delta t) \lfR{I}\rf{M}
\label{eq_qq}    
\end{equation}

\begin{equation}
\lf{W}\theta\rf{M}(t) = \Log (\lfR{W}\rf{M}(t))
\label{eq_qq}    
\end{equation}

\begin{equation}
\lf{M}\theta\rf{I} = \Log (\lfR{M}\rf{I})
\label{eq_qq}    
\end{equation}

parameters to estimate on the first stage

$\lf{W}\theta\rf{M}(0), \lf{M}\theta\rf{I}, b(t), M, A$

TOTHINK: $\lf{W}\theta\rf{M}(0)$ can be chosen right from master data

Freezing all the parameters on the second stage

$\lf{W}\theta\rf{M}(0'), \lf{M}\theta\rf{I}, b(t) = b(0'), M, A$

Functional to be minimized is the following

\begin{equation}
\mathcal{L} = \sum_{k=0}^K \left\| \Log (\lfR{W}\rf{M}(t_k) \lfR{M}\rf{W ref}(t_k)) \right\|_{\Sigma_{\theta}}^2 + \sum_{n=0}^N \left\| \Delta b_\omega(t_n) \right\|_{\Sigma_{b}}^2
\label{eq_qq}    
\end{equation}

\begin{equation}
\Delta b_\omega(t_n) = b_\omega(t_{n+1}) - b_\omega(t_n)
\label{eq_qq}    
\end{equation}

====================================

\section{Rigid Body Transformations}\label{sec_rbt}

Assume rigid-body platform where IMU-sensor is placed. IMU has its own frame I. Any frame M rigidly connected with the platform has constant displacement and orientation wrt. frame I. M stands for Master that can be any sensor namely visual camera, depth camera, lidar or any other essential point on the platform. This transformation between rigidly connected frames M and I can be expressed through transformation matrix $\lfT{I}\rf{M}$ such that pose of Master in global frame $\lfT{W}\rf{M}$ can be expressed via pose of IMU in global frame $\lfT{W}\rf{I}$ by following equation. 


\textbf{Zeroth derivative}
\begin{align*}
&& \lfT{W}\rf{M} &= \lfT{W}\rf{I} \lfT{I}\rf{M}\\
\\
\text{Expansion}
&& \lfR{W}\rf{M} &= \lfR{W}\rf{I} \lfR{I}\rf{M}\\
&& \lfp{W}\rf{M} &= \lfR{W}\rf{I} \lfp{I}\rf{M} + \lfp{W}\rf{I}
\end{align*}

Moreover the first and second derivatives of this connection give the following results.

\textbf{First derivative}

\begin{align*}
&& \lfdotT{W}\rf{M} &= \lfdotT{W}\rf{I} \lfT{I}\rf{M}\\
\\
\text{Expansion} && \lfR{W}\rf{M} [\lf{M}\omega]_\times &= \lfR{W}\rf{I} [\lf{I}\omega]_\times \lfR{I}\rf{M}\\
&& \lfR{W}\rf{M} \lf{M}v &= \lfR{W}\rf{I} ([\lf{I}\omega]_\times \lfp{I}\rf{M} + \lf{I}v)\\
\\
\text{Note 1} && [\lf{M}\omega]_\times &= \lfR{M}\rf{I} [\lf{I}\omega]_\times \lfR{I}\rf{M}\\
\text{or} && \lf{M}\omega &= \lfR{M}\rf{I} \lf{I}\omega\\
\text{Note 2} && \lf{M}v &= \lfR{M}\rf{I} ([\lf{I}\omega]_\times \lfp{I}\rf{M} + \lf{I}v)
\end{align*}

\textbf{Second derivative}
\begin{align*}
&& \lfddotT{W}\rf{M} &= \lfddotT{W}\rf{I} \lfT{I}\rf{M}\\
\\
\text{Ex}
&& \lfR{W}\rf{M} ([\lf{M}\omega]_\times^2 + [\lf{M}\dot{\omega}]_\times) &= \lfR{W}\rf{I} ([\lf{I}\omega]_\times^2 + [\lf{I}\dot{\omega}]_\times) \lfR{I}\rf{M}\\
%& & \lfR{W}\rf{M} ([\lf{M}\omega]_\times \lf{M}v + \lf{M}a) &= \lfR{W}\rf{I} \{([\lf{I}\omega]_\times^2 + [\lf{I}\dot{\omega}]_\times) \lfp{I}\rf{M} + [\lf{I}{\omega}]_\times \lf{I}v + \lf{I}a\}\\
&& \lfR{W}\rf{M} \lf{M}a &= \lfR{W}\rf{I} \{([\lf{I}\omega]_\times^2 + [\lf{I}\dot{\omega}]_\times) \lfp{I}\rf{M} + \lf{I}a\}\\
\\
\text{Note 1}
&& [\lf{M}\omega]_\times^2 + [\lf{M}\dot{\omega}]_\times &= \lfR{M}\rf{I} ([\lf{I}\omega]_\times^2 + [\lf{I}\dot{\omega}]_\times) \lfR{I}\rf{M}\\
\text{or} && \lf{M}\dot\omega &= \lfR{M}\rf{I} \lf{I}\dot\omega\\
\text{Note 2} && \lf{M}a &= \lfR{M}\rf{I} \{([\lf{I}\omega]_\times^2 + [\lf{I}\dot{\omega}]_\times) \lfp{I}\rf{M} + \lf{I}a\}\\
\end{align*}

But what is $\lfR{W}\rf{M}(t)$

\begin{equation}
\lf{M}\omega = \lfR{M}\rf{I}\lf{I}\omega
\label{eq_qq}
\end{equation}

=======================
\section{State variables and Frames}\label{sec_frames}

% 
The input variables are the readings from the IMU sensor, i.e., acceleration $a$ and angular velocity $\omega$ each of them measuring their corresponding variables in three axis.
The state variables are position $p \in \mathbb{R}^3$, orientation $\theta \in SO(3)$, velocity $v \in \mathbb{R}^3$ and the corresponding bias to the accelerometer $b_a$ and bias for the gyroscope $b_{\omega}$ 
=========================

\section{MIMU auction}

Suppose we want to utilize measurements from different imus represented in Master frame.

equations



For any rot m and omega belonging to SO3/so3

\begin{align}
\Exp (R \theta) = R \Exp (\theta) R^\top
\label{eq_qq}
\end{align}


\begin{equation}
\lfR{W}\rf{M}(t+\Delta t) = \lfR{W}\rf{M}(t) \Exp (\lf{M}\omega(t) \Delta t)
\label{eq_qq}
\end{equation}

\begin{equation}
\lfR{W}\rf{M}(t+\Delta t) = \lfR{W}\rf{M}(t) \lfR{M}\rf{I} \Exp (\lf{I}\omega(t) \Delta t) \lfR{I}\rf{M}
\label{eq_qq}    
\end{equation}

\begin{equation}
\lf{W}\theta\rf{M}(t) = \Ln (\lfR{W}\rf{M}(t))
\label{eq_qq}    
\end{equation}

\begin{equation}
\lf{M}\theta\rf{I} = \Ln (\lfR{M}\rf{I})
\label{eq_qq}    
\end{equation}

parameters to estimate on the first stage

$\lf{W}\theta\rf{M}(0), \lf{M}\theta\rf{I}, b(t), M, A$

TOTHINK: $\lf{W}\theta\rf{M}(0)$ can be chosen right from master data

Freezing all the parameters on the second stage

$\lf{W}\theta\rf{M}(0'), \lf{M}\theta\rf{I}, b(t) = b(0'), M, A$

Functional to be minimized is the following

\begin{equation}
\mathcal{L} = \sum_{k=0}^K \left\| \Ln (\lfR{W}\rf{M}(t_k) \lfR{M}\rf{W ref}(t_k)) \right\|_{\Sigma_{\theta}}^2 + \sum_{n=0}^N \left\| \Delta b_\omega(t_n) \right\|_{\Sigma_{b}}^2
\label{eq_qq}    
\end{equation}

\begin{equation}
\Delta b_\omega(t_n) = b_\omega(t_{n+1}) - b_\omega(t_n)
\label{eq_qq}    
\end{equation}


where $t_k$ timestamp of every IMU sample, $t_n$ is timestamp (HOWTO explain)

We model biases as piece-wise constant ones in relatively long horizon. Bias is constant within 30-samples period.

number of parameters for single IMU system

1 Sample: 3+3+6+3+9 = 24

h samples (constant bias horizon): (3+3)*h+6+3+9 = 

h*l samples: 3(2h+1)l + 15


% Cost function

Batch optimization of this factors. \TODO{}

=================================
Briefly:\\
\cite{olson2011apriltag} - AprilTag CITED\\
\cite{titterton2004strapdown} - common gyro and acc model. strapdown CITED\\
\cite{forster2015imu} - preintegration on manifold CITED\\
\cite{furgale2013} - Unified Temporal and Spatial Calibration for Multi-Sensor Systems\\
\cite{kevin2017modern} - RB-kinematics, book CITED\\
\cite{wuest2019online} and \cite{svacha2018inertial} and \cite{svacha2019inertial} - VN/VIN + drag forces model\\
\cite{nikolic2016characterisation} (\cite{nikolic2015maximum}) - Noise model / extrinsic and intrinsic parameters / device / application (thesis by Nikolic)\\
\cite{sola2018micro} - A micro Lie Theory\\
\cite{furgale2012continuous} - continuous time optimisation by splines. Before Kalibr CITED\\
\cite{moakher2002means} - means and averaging in groups of rotations\\
\cite{huang2019visual} - Visual-inertial navigation: A concise review. Tightly-Loosely coupled and other info\\
\cite{nilsson2016inertial} and \cite{skog2016inertial} - MIMU! Inertial sensor arrays. Review with equation or filters frameworks. Higher accuracy Higher reliability and uncertainties estimation Higher dynamic measurement range Estimation of angular motion from accelerometer data Direct estimation of angular acceleration\\
\cite{skog2014open} - MIMU! platform. To detect and isolate sensor failures, thereby
increasing the reliability and integrity of the sensor system.\\
\cite{skog2006calibration} - calibration of MEMS IMU\\
TORECALL \cite{d2018calibration1} and \cite{d2018calibration2} calibration of MEMS IMU\\
\cite{solin2018inertial} - inertial odometry using iphone and zero-velocity updates and
pseudo-measurements limiting the momentary speed algorithm\\
\cite{rehder2017camera} - camera/imu calibration revisited. Kalibr, the same hw sensor\\
\cite{rhudy2012fusion} - two fusion methods of GPS and Redundant IMU Data\\
\cite{eckenhoff2019multi} - Multi-Camera Visual-Inertial Navigation with Online Intrinsic and Extrinsic Calibration cam intr and both extr\\
TOREAD \cite{kim2017line} - On-Line Initialization and Extrinsic Calibration of an Inertial Navigation System With a Relative Preintegration Method on Manifold\\
\cite{eckenhoff2019sensor} - MIMU! Sensor-Failure-Resilient Multi-IMU Visual-Inertial Navigation\\
\cite{leutenegger2015keyframe} - Keyframe-Based Visual-Inertial Odometry UsingNonlinear Optimization to mention optimization instead of *KF methods\\
\cite{zhang2019lightweight} - MIMU! trials to improve accuracy by averaging MIMU measurements\\
\cite{crassidis2006sigma} - discrete model of bias explanation\\
\cite{rehder2016extending} - Kalibr\\
\cite{wang2019optimized} - Optimized Multi-Position Calibration Method with Nonlinear Scale Factor for Inertial Measurement Units\\
\cite{barfoot2017} - State Estimation for Robotics, Barfoot book\\


\cite{nilsson2016inertial} and \\
OK\cite{skog2016inertial} - MIMU! Inertial sensor arrays. Review with equation or filters frameworks. Higher accuracy Higher reliability and uncertainties estimation Higher dynamic measurement range Estimation of angular motion from accelerometer data Direct estimation of angular acceleration\\
OK\cite{skog2014open} - MIMU! platform. To detect and isolate sensor failures, thereby
increasing the reliability and integrity of the sensor system.\\
OK\cite{eckenhoff2019sensor} - MIMU! Sensor-Failure-Resilient Multi-IMU Visual-Inertial Navigation\\
OK\cite{zhang2019lightweight} - MIMU! trials to improve accuracy by averaging MIMU measurements\\
OK\cite{rhudy2012fusion} - three fusion methods of GPS and Redundant IMU Data\\
OK\cite{wang2019optimized} - Optimized Multi-Position Calibration Method with Nonlinear Scale Factor for Inertial Measurement Units\\
TOINTRO\cite{huang2019visual} - Visual-inertial navigation: A concise review. Tightly-Loosely coupled and other info\\
NOTNEEDED \cite{d2018calibration1} and \cite{d2018calibration2} calibration of MEMS IMU\\
\cite{rehder2016extending} - Kalibr\\
===============================


==> _pres.tex <==
\section{Formulas for Presentation}%\label{}

\begin{align}
    \pmb{p} (t) =& \int_0^t \int_0^t \pmb{a}(t') dt'^2\\
    \pmb{\theta}(t) =& \int_0^t \pmb{\omega}(t') dt'\\
\end{align}

\begin{align}
    \ac \neq & \; \ac_I\\
    \om \neq & \; \om_I\\
\end{align}

\begin{align}
    \ac = & \; R \, \ac_I\\
    \om = & \; R \, \om_I\\
    R = & \, \Exp(\pmb{\theta}) \in SO(3)
\end{align}

\begin{align}
    \ac_I \neq & \; \tilde \ac_I\\
    \om_I \neq & \; \tilde \om_I
\end{align}

\begin{align}
    \ac_I(t) = & \; A_a \tilde \ac_I(t) + \pmb{b}_a(t) + \pmb{\eta}_a(t)\\
    \om_I(t) = & \; A_\omega \tilde \om_I(t) + \pmb{b}_\omega(t) + \pmb{\eta}_\omega(t)
\end{align}
%b
\begin{align}
    \dot{\pmb{b}}_a(t) = & \; \pmb{\nu}_a(t)\\
    \dot{\pmb{b}}_\omega(t) = & \; \pmb{\nu}_\omega(t)
\end{align}

%\begin{align}
%    \ac_I(t_k) = & \; A_a \tilde \ac_I(t_k) + \pmb{b}_a(t_k) + \pmb{\eta}_a(t_k)\\
%    \om_I(t_k) = & \; A_\omega \tilde \om_I(t_k) + \pmb{b}_\omega(t_k) + \pmb{\eta}_\omega(t_k)
%\end{align}
%bd
%\begin{align}
%    \pmb{b}_a(t_k) = \pmb{b}_a(t_{k-1}) + \pmb{\nu}_a(t_k)\\
%    \pmb{b}_\omega(t_k) = \pmb{b}_\omega(t_{k-1}) + \pmb{\nu}_\omega(t_k)
%\end{align}

\begin{align}
    \ac_{I k} &= A_a \tilde \ac_{I k} + \pmb{b}_{a k} + \pmb{\eta}_{a k}\\
    \om_{I k} &= A_\omega \tilde \om_{I k} + \pmb{b}_{\omega k} + \pmb{\eta}_{\omega k}
\end{align}
%bd
\begin{align}
    \pmb{b}_k^a &= \pmb{b}_{k-1}^a + \pmb{\nu}_k^a\\
    \pmb{b}_k^\omega &= \pmb{b}_{k-1}^\omega + \pmb{\nu}_k^\omega
\end{align}

%\begin{align}
%    R(t_{k+1}) &= R(t_k) \Exp(\pmb{\omega}_I(t_k) \Delta t)\\
%    \pmb{v}(t_{k+1}) &= \pmb{v}(t_k) + R(t_k) \: \pmb{a}_I(t_k) \Delta t\\
%    \pmb{p}(t_{k+1}) &= \pmb{p}(t_k) + \pmb{v}(t_k)\Delta t + R(t_k) \: \pmb{a}_I(t_k) \Delta t^2/2\\
%\end{align}
\begin{align}
    R_{k+1} &= R_k \Exp(\pmb{\omega}_{I k} \Delta t)\\
    \pmb{v}_{k+1} &= \pmb{v}_k + R_k \: \pmb{a}_{I k} \Delta t\\
    \pmb{p}_{k+1} &= \pmb{p}_k + \pmb{v}_k\Delta t + R_k \: \pmb{a}_{I k} \; \Delta t^2/2\\
\end{align}
$\chi = \{
    R_k,
    \pmb{v}_k,
    \pmb{p}_k,
    \pmb{b}_k^a,
    \pmb{b}_k^\omega
    \: | \; k=1..N
\}$\\
\\

$$\chi* = \arg \min_\chi \log \mathcal{L}$$\\
\\
$\log \mathcal{L} = \sum_{k=1}^N \log \mathcal{L}_k$\\
\\
$\log \mathcal{L}_k = \|\Delta R_k\|_{\Sigma_R}^2 + \|\Delta \pmb{v}_k\|_{\Sigma_{\pmb{v}}}^2 + \|\Delta \pmb{p}_k\|_{\Sigma_{\pmb{p}}}^2 + \|\Delta \pmb{b}_k^a \|_{\Sigma_{\pmb{b}_k^a}}^2 + \|\Delta \pmb{b}_k^\omega \|_{\Sigma_{\pmb{b}_k^\omega}}^2$\\
\\
\begin{align}
    \Delta \pmb{v}_k &= \pmb{v}_k - \pmb{v}_k^{ref}\\
    \Delta \pmb{p}_k &= \pmb{p}_k - \pmb{p}_k^{ref}\\
    \Delta R_k &= R_k - R_k^{ref}\\
    \Delta \pmb{b}_k &= \pmb{b}_k-\pmb{b}_{k-1}
\end{align}
\\
$\log \mathcal{L} = \sum_{i=1}^M \sum_{k=1}^N \log \mathcal{L}_k^i + \mathcal{R}_k$\\
\\
$\mathcal{R}_k = \| \pmb{p}_k^A - \pmb{p}_k^B - \pmb{p}_k^{AB}\|_{\Sigma_{p}}^2 + \| \Ln((R_k^A)^T R_k^B R_k^{AB})\|_{\Sigma_{R}}^2 + \dots$\\
\\

Model:
$$a_I(t_k) = A_a \amk + b_a(t_k) + \eta_a(t_k),\hspace*{8pt} b_a(t_k + \Delta t) = b_a(t_k) + \nu_a(t_k)$$
$$\omega_I(t_k) = A_\omega \omk + b_\omega(t_k) + \eta_\omega(t_k),\hspace*{8pt} b_\omega(t_k) = b_\omega(t_k)  + \nu_\omega(t_k)$$\\
\\
Exponent map
skatch\\
\\
$R = \Exp(\theta)$\\
\\
\\
$v(t_0) = v_0,\hspace*{4pt} r(t_0) = r_0,\hspace*{4pt} R(t_0) = R_0$\\
\\
$R(t_{k} + \Delta t) = R(t_k) \Exp(\omega_I(t_k) \Delta t)$\\
\\
$v(t_{k} + \Delta t ) = v(t_k) + R(t_k) \: a_I(t_k) \Delta t$\\
\\
$r(t_{k} + \Delta t) = r(t_k) + v(t_k)\Delta t + R(t_k) \: a_I(t_k) \Delta t^2/2$\\
\\
%$\theta_I(t_{k+1}) = \Ln(R(t_{k+1}))$
\\
Parameters\\
\\
$\chi = \{r(t_k), v(t_k), R(t_k), b_a (t_k), b_\omega(t_k)\}$\\
\\
$$\chi* = \arg \min_\chi \log \mathcal{L}$$\\
Factors\\
\\
$\log \mathcal{L} = \sum_{k=1}^N \log \mathcal{L}_k$\\
\\
$\log \mathcal{L}_k = \|\Delta r(t_k)\|_{\Sigma_r}^2 + \|\Delta v(t_k)\|_{\Sigma_v}^2 + \|\Delta R_k\|_{\Sigma_R}^2 + \|\Delta b_a (t_k)\|_{\Sigma_{b_a}}^2 + \|\Delta b_\omega (t_k)\|_{\Sigma_{b_g}}^2$\\
\\
$\Delta r(t_k) = r(t_k) - r_{ref}(t_k)$\\
\\
$\Delta v(t_k) = v(t_k) - v_{ref}(t_k)$\\
\\
$\Delta R(t_k) = \Ln(R^T(t_k) R_{ref}(t_k))$\\
\\
$\Delta b_a (t_k) = b_a(t_k)-b_a(t_{k-1})$\\
\\
$\Delta b_\omega (t_k) = b_\omega(t_k)-b_\omega(t_{k-1})$\\
\\
RB\\
\\
$0 = r_B - (r_A + r_{AB})$\\
%\\
$I = R_B^T R_A R_{AB}$\\
%\\
$0 = v_B - (v_A + f(r_{AB}, \omega_A, \omega_B))$\\
%\\
$0 = \omega_B - h(\omega_A, R_{AB})$\\
%\\
$0 = a_B - (a_A + g(r_{AB}, v_a, v_b, \omega_A, \omega_B, R_{AB}))$\\
\\
$r_I(t), \theta_I(t)$\\
\\
$\am, \om$\\
\\
$\pmb{\omega} = \frac{d\pmb{\theta}}{dt}$\\
\\
$\pmb a = \frac{d^2 \pmb{p}}{dt^2}$\\


$\Delta \pmb{\theta} = \Ln (\Exp(\pmb{\theta}_1)^T\Exp(\pmb{\theta}_2))$\\
\\
$\Delta \pmb{\theta} = \pmb{\theta}_2 - \pmb{\theta}_1$\\
\\
$R \in SO(3)$\\
\\
$\pmb{\theta}^{\wedge} = \begin{bmatrix}
0 & -\theta_z & \theta_y\\
\theta_z & 0 & -\theta_x\\
-\theta_y & \theta_x & 0
\end{bmatrix}$\\
\\
$\Exp(\pmb{\theta})$\\
\\
$\exp(\pmb{\theta}^{\wedge})$\\
\\
$\Ln(R)$\\
\\
$\ln(R)$\\
\\
$\pmb{\theta}^{\wedge}$\\
\\
$(\pmb{\theta}^{\wedge})^{\vee}$\\
\\
$R$\\
\\
$\pmb{\theta}$\\
\\
$\pmb{\theta}^{\wedge}$\\
\\
$R \dot R = \pmb{\omega}^{\wedge}$\\
\\
$R_{k+1} = \Exp(\theta_k + \pmb{\omega}_{I k} \Delta t)$\\
\\
$\pmb{p}_A - \pmb{p}_B - R_B \pmb{p}_{AB}$\\
\\
$\Ln(R_A^T R_B R_{BA})$\\
\\
$R_A \pmb{v}_A - R_B (\oh_B \; \pmb{p_{BA}} + \pmb{v}_B)$\\
\\
$\Ln((R_A \oh_A)^T R_B \oh_B R_{BA})$\\
\\
$R_A (\oh_A\pmb{v}_A + \pmb{a}_A) - R_B (\fob \pmb{p}_{BA} + \oh_B \pmb{v}_B + \pmb{a}_B)$\\
\\
$\Ln((R_A \foa)^T R_B \fob R_{BA})$\\
\\
\begin{align*}
    \mathcal{R} &= \| \pmb{p}_A - \pmb{p}_B - R_B \pmb{p}_{AB} \|_{\Sigma_{p}}^2 &(p)\\
    &+ \| \Ln(R_A^T R_B R_{BA}) \|_{\Sigma_{\theta}}^2 &(\theta)\\
    &+ \| R_A \pmb{v}_A - R_B (\oh_B \; \pmb{p_{BA}} + \pmb{v}_B) \|_{\Sigma_{v}}^2 &(v)\\
    &+ \| \Ln((R_A \oh_A)^T R_B \oh_B R_{BA}) \|_{\Sigma_{\omega}}^2 &(\omega)\\
    &+ \| R_A (\oh_A\pmb{v}_A + \pmb{a}_A) - R_B (\fob \pmb{p}_{BA} + \oh_B \pmb{v}_B + \pmb{a}_B) \|_{\Sigma_{a}}^2  &(a)\\
    &+ \| \Ln((R_A \foa)^T R_B \fob R_{BA}) \|_{\Sigma_{\dot \omega}}^2 &(\dot \omega)
\end{align*}

